FedCAPrivacy: Privacy-Preserving Heterogeneous Federated Learning with Anonymous Adaptive Clustering

Federated learning (FL) is a distributed machine learning paradigm enabling multiple clients to train a model collaboratively without exposing their local data. Among FL schemes, clustering is an effective technique addressing the heterogeneity issue (i.e., differences in data distribution and computational ability affect training performance and effectiveness) via grouping participants with similar computational resources or data distribution into clusters. However, intra-cluster data exchange poses privacy risks, while cluster selection and adaptation introduce challenges that may affect overall performance. To address these challenges, this paper introduces anonymous adaptive clustering, a novel approach that simultaneously enhances privacy protection and boosts training efficiency. Specifically, an oblivious shuffle-based anonymization method is designed to safeguard user identities and prevent the aggregation server from inferring similarities through clustering. Additionally, to improve performance, we introduce an iteration-based adaptive frequency decay strategy, which leverages variability in clustering probabilities to optimize training dynamics. With these techniques, we build the FedCAPrivacy; experiments show that FedCAPrivacy achieves ~7X improvement in terms of performance while maintaining high privacy.

==> sections/3ps.tex <==
\section{Problem Statement}
\label{sec:ps}

\subsection{Threat Model}

In this work, we focus on privacy and security vulnerabilities that could be abused by \textit{honest and curious} adversaries. 
We assume that each honest participant possesses a private dataset, and adversaries could be involved in training without a dataset.  
The servers are honestly following all the protocols while attempting to compromise the user's data privacy based on the data they receive.
Our proposed framework utilizes a two-server architecture, whereby data between the participant and the server is transmitted over a public channel, and the servers communicate with each other over a private channel. We assume that there is no collusion between all entities.

\subsection{Heterogeneity in FL}
Following the standard setup of FL given in~\ref{subsec:fl}, each participant has a private dataset $D=\{(X, Y)|X\in \mathbb{R}^{N\times I}, Y\in \mathbb{R}^{N\times O}\}$, where $N$ represents the number of data sample, $I$ denotes the input size and $O$ is defined as the number of class for classification~\cite{huang2022learn}. Moreover, in heterogeneous FL, data heterogeneity and device heterogeneity are defined below:
\begin{itemize}
    \item Heterogeneous Data: On the one hand, the label distributions $P(Y)$ may be different for different clients even if the label distribution is shared, \textit{i.e.}, $P_i(X|Y) = P_j(X|Y)$. On the other hand, even when the feature distribution $P(X)$ is consistent across clients, the label distribution may be different for different clients, \textit{i.e.}, $P_i(Y|X) \neq P_j(Y|X)$~\cite{ye2023heterogeneous}.
    \item Heterogeneous Device: Each client runs $E$ epochs of local-update stochastic gradient descent (SGD) with a mini-batch size $B$. Thus, the local iteration number for a client with $d$ local samples is $\lfloor \frac{Ed}{B}\rfloor$, which can vary widely between devices.
    
\end{itemize}

